Measurement of $\Lambda$ Polarization in the $\pi^{-}p \to K^{0} \Lambda$ Reaction at $p_{\pi^{-}}=1.33$ GeV/$c$ toward a New $\Lambda p$ Scattering Experiment

This paper presents high-precision experimental data of the polarization of the $\Lambda$ hyperon in the $\pi^{-}p \to K^{0} \Lambda$ reaction, measured in the angular range $0.6<\cos \theta ^{CM}_{K0}<1.0$ with a fine bin width of $d\cos \theta ^{CM}_{K0}=0.05$. The data were obtained from the J-PARC E40 experiment at the K1.8 beamline in the J-PARC Hadron Experimental Facility. The observed average polarization of $\Lambda$ in the range $0.60<\cos \theta ^{CM}_{K0}<0.85$ was $0.932 \pm 0.058 \,(\text{stat}) \pm 0.028 \,(\text{syst})$, demonstrating the successful extraction of precise polarization observables. This result provides essential experimental input for partial wave analysis (PWA) of dynamical coupled-channel (DCC) models, which aim to uncover the underlying mechanisms of $N^{*}$ resonances that emerge in intermediate states of $\pi N$ and $\gamma N$ interactions. Besides, it indicates the feasibility of a strongly polarized $\Lambda$ beam suitable for future $\Lambda p$ scattering experiments (e.g., J-PARC E86).

==> begin.tex <==
\makeatletter
\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

%%%%%%%%%  paragraph 設定 %%%%%%%%%%%
\makeatletter
\renewcommand{\paragraph}{%
  \@startsection{paragraph}%
   {4}%
   {\z@}%
   {0.5\Cvs \@plus.5\Cdp \@minus.2\Cdp}
   {-1zw}
   {\normalfont\normalsize\bfseries $\blacklozenge$\ }%
  % {\normalfont\normalsize\bfseries $\Diamond$\ }%
}%
\makeatother
%%%%%%%%%  paragraph 設定 %%%%%%%%%%%
\newcommand{\Lam}{\Lambda}
\newcommand{\Lp}{\Lambda p}
\newcommand{\PiKL}{\pi^-  p \to K^0 \Lambda}
\newcommand{\Kz}{K^{0}}
\newcommand{\KP}{K^{+}}
\newcommand{\KM}{K^{-}}
\newcommand{\KMstop}{K^{-}_{\rm stop}}
\newcommand{\costkz}{\cos{\theta^{K0}_{CM}}}
\newcommand{\Sp}{\Sigma p}

\newcommand{\BB}{{\rm B}_{8}{\rm B}_{8}}
\newcommand{\SM}{\Sigma^{-}}
\newcommand{\Sz}{\Sigma^{0}}
\newcommand{\SPp}{\Sigma^{+}p}
\newcommand{\SMp}{\Sigma^{-}p}
\newcommand{\SPMp}{\Sigma^{\pm}p}

\newcommand{\SMpLn}{\Sigma^- p \to \Lambda n}
\newcommand{\LN}{\Lambda N}
\newcommand{\pM}{\pi^{-}}
\newcommand{\pP}{\pi^{+}}
\newcommand{\Ldecay}{\Lambda \to p\pM}
\newcommand{\SN}{\Sigma N}
\newcommand{\PiKSM}{\pM p\to\KP\SM}
\newcommand{\PiKX}{\pM p\to\Kz X}
\newcommand{\kzdecay}{\Kz\to\pP\pM}
\newcommand{\mm}{M_{\PiKX}}

\newcommand{\costp}{\cos{\theta_p}}
\newcommand{\multipi}{\pi^-  p \to \pi^-\pi^-\pi^+p}
\newcommand{\dzkz}{\Delta z_{K^{0}}}
\newcommand{\dz}{\Delta z}
\newcommand{\costcm}{\cos{\theta}_{CM}}
\newcommand{\chisq}{\chi^{2}}
\newcommand{\mubg}{\mu_{BG}}
\newcommand{\dzupper}{\Delta z_{\Kz,\ Upper}}
\newcommand{\dzlower}{\Delta z_{\Kz,\ Lower}}

\newcommand{\dtheta}{\Delta\theta}

\newcommand{\accPL}{\epsilon_{P_{\Lam}}}
\newcommand{\erraccPL}{\sigma(\epsilon_{P_{\Lam}})}
\newcommand{\accPLi}{\epsilon_{P_{\Lam},\ i}}
\newcommand{\erraccPLi}{\sigma(\epsilon_{P_{\Lam},\ i})}

\newcommand{\com}[1]{{\bf \color{blue}#1}}
\newcommand{\fix}[1]{\color{black}#1}
\newcommand{\sfix}[1]{{\color{black}#1}}
\newcommand{\fixxx}[1]{\color{black}#1}
\newcommand{\fixxxx}[1]{\color{red}#1}
\newcommand{\wip}[1]{\color{black}#1}

